A multiple spacecraft detection of the 2 April 2022 M-class flare and filament eruption during the first close Solar Orbiter perihelion

The Solar Orbiter mission completed its first remote-sensing observation windows in the spring of 2022. On 2/4/2022, an M-class flare followed by a filament eruption was seen both by the instruments on board the mission and from several observatories in Earth's orbit. The complexity of the observed features is compared with the predictions given by the standard flare model in 3D. We use the observations from a multi-view dataset, which includes EUV imaging to spectroscopy and magnetic field measurements. These data come from IRIS, SDO, Hinode, as well as several instruments on Solar Orbiter. Information given by SDO/HMI and Solar Orbiter PHI/HRT shows that a parasitic polarity emerging underneath the filament is responsible for bringing the flux rope to an unstable state. As the flux rope erupts, Hinode/EIS captures blue-shifted emission in the transition region and coronal lines in the northern leg of the flux rope prior to the flare peak. Solar Orbiter SPICE captures the whole region, complementing the Doppler diagnostics of the filament eruption. Analyses of the formation and evolution of a complex set of flare ribbons and loops show that the parasitic emerging bipole plays an important role in the evolution of the flaring region. While the analysed data are overall consistent with the standard flare model, the present particular magnetic configuration shows that surrounding magnetic activity such as nearby emergence needs to be taken into account to fully understand the processes at work. This filament eruption is the first to be covered from different angles by spectroscopic instruments, and provides an unprecedented diagnostic of the multi-thermal structures present before and during the flare. This dataset of an eruptive event showcases the capabilities of coordinated observations with the Solar Orbiter mission.

==> labels.tex <==


1 Section \ref{sec-Introduction}
2 Section \ref{sec-Overview}
   2.1 Section \ref{sec-Longterm}
   2.2 Section \ref{sec-M-class}
   2.3 Section \ref{sec-Spectroscopic}   
3 Section \ref{sec-Precursor}
   3.1 Section \ref{sec-Flux_emergence}
   3.2 Section \ref{sec-Overlying}
   3.3 Section \ref{sec-Comparison}
4 Section \ref{sec-Eruption}
   4.1 Section \ref{sec-SPICE}
   4.2 Section \ref{sec-Filament}
   4.3 Section \ref{sec-Sources}
5 Section \ref{sec-Discussions}
6 Section \ref{sec-Conclusions}

Appendix 
A.
A.1\ref{eis_aia_alignement}
A.2\ref{los_radial_speeds}

 1 Fig.~\ref{solo-position}: shows the different FOVs of each instrument
 2 Fig.~\ref{overview-activeregions}: to explain the position of the two ARs and the region related to the filament
 3 Fig.~\ref{xrayflux}: GOES X ray light curves
 4 Fig.~\ref{imageurs-euv}: Overview of the eruption from the EUV imagers (AIA and EUI) + LASCO
 5 Fig.~\ref{iris}
 6 Fig.~\ref{goes_stix_lc}
 7 Fig.~\ref{magnetograms}
 Shows the evolution of the magnetograms
 8 Fig.~\ref{vnt-eis}
 EIS raster with Vnt
9 Fig.~\ref{hri-spice-loops-stackplots}
overlying loops
10 Fig.~\ref{aia-looptop}
early rise phase filament
11 Fig.~\ref{spice-intensities}
12 Fig.~\ref{spice-fexviiimaps}
13 Fig.~\ref{spice-doppler}

14 Fig.~\ref{fig.composite}
Intensity of He II (filament eruption) and Fe XXIV (flare loops)

15 Fig.~\ref{fig.movie1}
EIS and AIA comparison + cartoon
16 Fig.~\ref{fig.he2-twist}
Variation along the slit

17 Fig.~\ref{fig.multitemp}
18 Fig.~\ref{fig.eis-aia}
zoom on filament

% 19 Fig.~\ref{stix_spec}
19 Fig.~\ref{reconnection-diagram}

1 Table~\ref{table-Ions}
2 Table \ref{table-features}


